Augmenting Neural Networks with Priors on Function Values

The need for function estimation in label-limited settings is common in the natural sciences. At the same time, prior knowledge of function values is often available in these domains. For example, data-free biophysics-based models can be informative on protein properties, while quantum-based computations can be informative on small molecule properties. How can we coherently leverage such prior knowledge to help improve a neural network model that is quite accurate in some regions of input space -- typically near the training data -- but wildly wrong in other regions? Bayesian neural networks (BNN) enable the user to specify prior information only on the neural network weights, not directly on the function values. Moreover, there is in general no clear mapping between these. Herein, we tackle this problem by developing an approach to augment BNNs with prior information on the function values themselves. Our probabilistic approach yields predictions that rely more heavily on the prior information when the epistemic uncertainty is large, and more heavily on the neural network when the epistemic uncertainty is small.

==> tables_orig.tex <==
\begin{table*}[h!]
\caption{Results on avGFP fluorescence prediction.Plus-minus indicates the standard error computed from 10 train-test splits of the data.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lllll}
\toprule
           Method &   Log Likelihood &            RMSE &             MAE &            NDCG \\
\midrule
               NN & $-7.92 \pm 0.61$ & $1.05 \pm 0.01$ & $0.72 \pm 0.01$ & $0.97 \pm 0.00$ \\
         Stacking & $-8.39 \pm 0.40$ & $1.05 \pm 0.01$ & $0.72 \pm 0.01$ & $0.97 \pm 0.00$ \\
              BNN & $-5.63 \pm 0.21$ & $1.03 \pm 0.01$ & $0.70 \pm 0.01$ & $0.97 \pm 0.00$ \\
\ourmodel\ \constprior & $-1.82 \pm 0.00$ & $0.98 \pm 0.01$ & $0.66 \pm 0.01$ & $0.98 \pm 0.00$ \\
\ourmodel\ \rosettaprior & $-1.52 \pm 0.01$ & $0.85 \pm 0.02$ & $0.56 \pm 0.01$ & $0.98 \pm 0.00$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


\begin{table*}[h!]
\caption{Results on GB1 binding affinity prediction. Plus-minus indicates the standard error computed from 10 train-test splits of the data.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lllll}
\toprule
             Method &   Log Likelihood &            RMSE &             MAE &            NDCG \\
\midrule
                 NN & $-0.96 \pm 0.05$ & $0.62 \pm 0.03$ & $0.44 \pm 0.02$ & $0.78 \pm 0.01$ \\
           Stacking & $-0.94 \pm 0.05$ & $0.60 \pm 0.03$ & $0.45 \pm 0.03$ & $0.80 \pm 0.01$ \\
                BNN & $-0.80 \pm 0.02$ & $0.54 \pm 0.01$ & $0.38 \pm 0.01$ & $0.81 \pm 0.01$ \\
  \ourmodel\ \constprior & $-0.80 \pm 0.01$ & $0.53 \pm 0.01$ & $0.38 \pm 0.01$ & $0.81 \pm 0.01$ \\
\ourmodel\ \rosettaprior & $-0.56 \pm 0.00$ & $0.36 \pm 0.00$ & $0.11 \pm 0.00$ & $0.81 \pm 0.01$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


\begin{table*}[h!]
\caption{Results on blah, blah. Plus-minus indicates the standard error computed from 10 train-test splits of the data.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lllll}
\toprule
       Method &   Log Likelihood &            RMSE &             MAE &        Spearman \\
\midrule
          SFI & $-2.09 \pm 0.00$ & $1.86 \pm 0.00$ & $1.41 \pm 0.00$ & $0.73 \pm 0.00$ \\
           NN & $-2.40 \pm 0.05$ & $1.90 \pm 0.03$ & $1.34 \pm 0.02$ & $0.75 \pm 0.01$ \\
     Stacking & $-2.30 \pm 0.03$ & $1.12 \pm 0.01$ & $1.22 \pm 0.01$ & $0.77 \pm 0.00$ \\
          BNN & $-2.06 \pm 0.01$ & $1.73 \pm 0.02$ & $1.16 \pm 0.01$ & $0.78 \pm 0.00$ \\
\ourmodel\ SFI Prior & $-2.04 \pm 0.01$ & $1.68 \pm 0.01$ & $1.12 \pm 0.01$ & $0.79 \pm 0.00$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}








